Speech Prefix-Tuning with RNNT Loss for Improving LLM Predictions

In this paper, we focus on addressing the constraints faced when applying LLMs to ASR. Recent works utilize prefixLM-type models, which directly apply speech as a prefix to LLMs for ASR. We have found that optimizing speech prefixes leads to better ASR performance and propose applying RNNT loss to perform speech prefix-tuning. This is a simple approach and does not increase the model complexity or alter the inference pipeline. We also propose language-based soft prompting to further improve with frozen LLMs. Empirical analysis on realtime testset from 10 Indic languages demonstrate that our proposed speech prefix-tuning yields improvements with both frozen and fine-tuned LLMs. Our recognition results on an average of 10 Indics show that the proposed prefix-tuning with RNNT loss results in a 12\% relative improvement in WER over the baseline with a fine-tuned LLM. Our proposed approches with the frozen LLM leads to a 31\% relative improvement over basic soft-prompting prefixLM.

==> figures/tikz/one.tex <==
\begin{axis}[
    xlabel={n},
    ylabel={$S_{400}(8,n)$}
    xmin=1,
    xmax=5,
    xtick={1,2,3,4,5},
    xticklabels={1,2,3,4,5},
    ymin=40,
    ymax=100,
    legend pos=south east,
    legend style = {nodes = {scale=0.85, transform shape},
    % legend columns=2
    }
]
    \addplot[color=magenta, mark=x]
    coordinates {
        (1, 70.46)
        (2, 78.8)
        (3, 82.53)
        (4, 84.28)
        (5, 85.02)
    };
    \addlegendentry{Baseline}
    \addplot[color=teal, mark=+]
    coordinates {
        (1, 71.37)
        (2, 77.58)
        (3, 81.27)
        (4, 83.41)
        (5, 84.46)
    };
    \addlegendentry{HypOnly}
    \addplot[color=violet, mark=square]
    coordinates {
        (1, 58.17)
        (2, 69.5)
        (3, 74.79)
        (4, 78.33)
        (5, 80.59)
    };
    \addlegendentry{FixedLengthAudio}
    % \addplot[color=red, mark=triangle]
    \addplot[color=blue, mark=o]
    coordinates {
        (1, 58.46)
        (2, 69.53)
        (3, 74.73)
        (4, 77.76)
        (5, 80.27)
    };
    \addlegendentry{FLA+Multitask}
\end{axis}

% weights = [(1, 1738), (2, 2734), (3, 3562), (4, 4397), (5, 5275)]

==> figures/tikz/one_abs.tex <==
\begin{axis}[
    xlabel={n},
    ylabel={$S_{400}(8,n)$}
    xmin=1.5,
    xmax=5,
    xtick={1,2,3,4,5},
    xticklabels={1,2,3,4,5},
    ymin=40,
    ymax=100,
    legend pos=south east,
    legend style = {nodes = {scale=0.85, transform shape},
    % legend columns=2
    }
]
    \addplot[color=magenta, mark=x]
    coordinates {
        (1, 70.46)
        (2, 91.85)
        (3, 94.85)
        (4, 91.75) 
        (5, 88.73)
    };
    \addlegendentry{Baseline}
    \addplot[color=teal, mark=+]
    coordinates {
        (1, 71.37)
        (2, 88.41)
        (3, 93.45) 
        (4, 92.53)
        (5, 89.72)
    };
    \addlegendentry{HypOnly}
    \addplot[color=violet, mark=square]
    coordinates {
        (1, 58.17)
        (2, 89.27)
        (3, 92.26)
        (4, 93.43)
        (5, 91.91)
    };
    \addlegendentry{FixedLengthAudio}
    % \addplot[color=red, mark=triangle]
    \addplot[color=blue, mark=o]
    coordinates {
        (1, 58.46)
        (2, 88.85)
        (3, 91.90)
        (4, 90.69) 
        (5, 92.84)
    };
    \addlegendentry{FLA+Multitask}
\end{axis}

% weights = [(1, 1738), (2, 2734), (3, 3562), (4, 4397), (5, 5275)]

% (1, 58.17)
%         (2, 69.5)
%         (3, 74.79)
%         (4, 78.33)
%         (5, 80.59)
%     };
%     \addlegendentry{FixedLengthAudio}
%     % \addplot[color=red, mark=triangle]
%     \addplot[color=blue, mark=o]
%     coordinates {
%         (1, 58.46)
%         (2, 69.53)
%         (3, 74.73)
%         (4, 77.76)
%         (5, 80.27)

==> figures/tikz/two.tex <==
\begin{semilogxaxis}[
    xlabel={n},
    ylabel={$S_{400}(k,1)$}
    xmin=1,
    xmax=8,
    xtick={1,2,4,8},
    xticklabels={1,2,4,8},
    ymin=40,
    ymax=100,
    legend pos=south east,
    legend style = {nodes = {scale=0.85, transform shape},
    % legend columns=2
    }
]
    \addplot[color=magenta, mark=x]
    coordinates {
        % (1, 70.46)
        % (2, 78.8)
        % (3, 82.53)
        % (4, 84.28)
        % (5, 85.02)
        (1, 85.36)
        (2, 78.93)
        (4, 75.47)
        (8, 70.46)
    };
    \addlegendentry{Baseline}
    \addplot[color=teal, mark=+]
    coordinates {
        % (1, 71.37)
        % (2, 77.58)
        % (3, 81.27)
        % (4, 83.41)
        % (5, 84.46)
        (1, 89.76)
        (2, 81.15)
        (4, 75.88)
        (8, 71.37)
    };
    \addlegendentry{HypOnly}
    \addplot[color=violet, mark=square]
    coordinates {
        % (1, 58.17)
        % (2, 69.5)
        % (3, 74.79)
        % (4, 78.33)
        % (5, 80.59)
        (1, 82.97)
        (2, 71.92)
        (4, 63.98)
        (8, 58.17)
    };
    \addlegendentry{FixedLengthAudio}
    % \addplot[color=red, mark=triangle]
    \addplot[color=blue, mark=o]
    coordinates {
        % (1, 58.46)
        % (2, 69.53)
        % (3, 74.73)
        % (4, 77.76)
        % (5, 80.27)
        (1, 81.88)
        (2, 70.54)
        (4, 64.04)
        (8, 58.46)
    };
    \addlegendentry{FLA+Multitask}
\end{semilogxaxis}

